Nonlinear response of 2DEG in the quantum Hall regime

Breaking of inversion symmetry leads to nonlinear and nonreciprocal electron transport, in which the voltage response does not invert with the reversal of the current direction. Many systems have incorporated inversion symmetry breaking into their band or crystal structures. In this work, we demonstrate that a conventional two-dimensional electron gas (2DEG) system with a back gate shows non-reciprocal behavior (with voltage proportional to current squared) in the quantum Hall regime, which depends on the out-of-plane magnetic field and contact configuration. The inversion symmetry is broken due to the presence of the back gate and magnetic field, and our phenomenological model provides a qualitative explanation of the experimental data. Our results suggest a universal mechanism that gives rise to non-reciprocal behavior in gated samples.

==> NotInUse/modelOLD.tex <==
\subsection{Model}
First, in the quantum Hall plateau ($B=B_{\textrm{Q}}$) regime, the current is carried by the edge channels and no dissipation occurs. Therefore, the potential distribution would look like the dotted lines shown in Fig. \ref{correlation}(b). $U(x, B)$ and $L(x, B)$ are the potential along the upper and the lower channel. In the Figure, $R_{xy}^{Q}$ is the Hall resistance at the quantum Hall plateau. The contacts along the upper channel separated by a distance $d$ see the voltage $V_{xx}(\textrm{upper})$, which is the potential difference between $U(x)$ and $U(x+d)$.
We suppose that the potential is given by the product of Hall resistivity $\rho_{xy}$ and the injected current $I$.
Then, $V_{xx}(\textrm{upper})$ is given by $V_{xx}(\textrm{upper})=U(x)-U(x+d)=R_{xy}^{Q}I/2-R_{xy}^{Q}I/2=0$. Similarly, the Hall voltage $V_{xy}(\textrm{left})$ is given by the voltage difference between the two contacts on the left or right side of the sample, $V_{xy}(\textrm{left})=U(x)-L(x)=R_{xy}^{Q}I/2-(-R_{xy}^{Q}I/2)=R_{xy}^{Q}I$. Note that both $V_{xx}(\textrm{upper})$ and $V_{xy}(\textrm{left})$ are linear in $I$. This agrees with the experimental observation that there is no non-linearity in the plateau regime.

Next, we consider the situation $B=B_{\textrm{Q}}+\delta B$, where $\delta B$ is the deviation in a magnetic field to make the system be outside the plateau. Then, the current is carried not only by the edge channel but also by the bulk, giving rise to a finite dissipation.
Now, the position-dependent potential can be written as $U(x)=\rho_{xy}(\textrm{top},x,n(x))I$. The $x$-dependence of $\rho_{xy}$ comes from the fact that the system is outside the plateau. The key assumption is that the carrier density is also a function of $x$, making $n(x)$. Considering that the carrier density is determined by the potential difference between the 2DEG and the back gate, $n(x)$ can be written as $n(x)=n_{0}+C\left[V_{\textrm{BG}}+T(x)\right]$. Here, $n_{0}$ is the carrier density without back gate voltage and the injection current, and $C$ is the capacitance between the 2DEG and the back gate. Then, $U(x)$ can be expressed as below.
\begin{equation}
\begin{split}
U(x)&=\rho_{xy}\left(\textrm{upper},x,n\left(x\right)\right)I\\
%&=\rho_{xy}\left(\textrm{upper},x,n_{0}+CV_{\textrm{BG}}+CT\left(x\right)\right)I\\
&\simeq\rho_{xy}\left(\textrm{upper},x,n_{0}+CV_{\textrm{BG}}\right)I+\frac{\partial\rho_{xy}}{\partial n}CT\left(x\right)I.
\end{split}
\label{Tx}
\end{equation}
Here, we assumed that the amount of modulation of the carrier density due to the injection current is small enough compared to the original carrier density ($CT\left(x\right)\ll n_{0}+CV_{\textrm{BG}}$).
The above equation can be solved with $U(x)$.
\begin{equation}
\begin{split}
U(x)&\simeq\frac{\rho_{xy}\left(\textrm{upper},x,n_{0}+CV_{\textrm{BG}}\right)I}{1-\frac{\partial\rho_{xy}}{\partial n}CI}\\
&\simeq\rho_{xy}^{\textrm{U}}(x)I+\rho_{xy}^{\textrm{U}}(x)\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}CI^{2},
\end{split}
\label{TxFinal}
\end{equation}
where $\rho_{xy}^{\textrm{U}}(x)=\rho_{xy}\left(\textrm{upper},x,n_{0}+CV_{\textrm{BG}}\right)$. We assumed that the amount of potential modulation due to the injection current is small enough compared to the total potential ($\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}CU(x)I\ll U(x)I$), which also means that the first term of Eq. (\ref{Tx}) is much larger than the second term.
Assuming a mild potential gradient, $U(x+d)\simeq U(x)+\frac{\partial U(x)}{\partial x}d$. This leads to the expression of $U(x+d)$.
\begin{equation}
\begin{split}
U(x+d)&\simeq U(x)+\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}dI\\
&+\left(\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}+\rho_{xy}^{\textrm{U}}(x)\frac{\partial^{2}\rho_{xy}^{\textrm{U}}(x)}{\partial n\partial x}\right)\\
&\times dCI^{2},
\end{split}
\label{TxFinal}   
\end{equation}


One can repeat a similar calculation for the lower channel and obtain the expression for $L(x)$.
\begin{equation}
L(x)\simeq\rho_{xy}^{\textrm{L}}(x)I+\rho_{xy}^{\textrm{L}}(x)\frac{\partial\rho_{xy}^{\textrm{L}}(x)}{\partial n}CI^{2},
\end{equation}
where $\rho_{xy}^{\textrm{L}}(x)=\rho_{xy}\left(\textrm{lower},x,n_{0}+CV_{\textrm{BG}}\right)$.

Now that we have $U(x)$ and $L(x)$, we use them to express $V_{xx}(\textrm{upper})$ and $V_{xx}(\textrm{left})$.
\begin{equation}
\begin{split}
V_{xx}(\textrm{upper})&\simeq -\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}dI\\
&-\left(\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}+\rho_{xy}^{\textrm{U}}(x)\frac{\partial^{2}\rho_{xy}^{\textrm{U}}(x)}{\partial n\partial x}\right)\\
&\times dCI^{2}
\end{split}
\label{Vxx}
\end{equation}
%
%
\begin{equation}
\begin{split}
V_{xy}(\textrm{upper})&=U(x)-L(x)\\
&=\left(\rho_{xy}^{\textrm{U}}(x)-\rho_{xy}^{\textrm{L}}(x)\right)I\\
&+\left(\rho_{xy}^{U}(x)\frac{\partial\rho_{xy}^{\textrm{U}}}{\partial n}-\rho_{xy}^{L}(x)\frac{\partial\rho_{xy}^{\textrm{L}}(x)}{\partial n}\right)CI^{2}
\end{split}
\label{Vxy}
\end{equation}

The linear and nonlinear resistances are derived from the above expression.
\begin{equation}
\begin{split}
R_{xx}&=-\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}d\\
R_{xy}&=\rho_{xy}^{\textrm{U}}(x)-\rho_{xy}^{\textrm{L}}(x)
\end{split}
\label{linear resistance}
\end{equation}
\begin{equation}
\begin{split}
R_{xx}^{(2)}(\textrm{upper})&=-2\left(\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial x}\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}+\rho_{xy}^{\textrm{U}}(x)\frac{\partial^{2}\rho_{xy}^{\textrm{U}}(x)}{\partial n\partial x}\right)dC\\
R_{xy}^{(2)}(\textrm{left})&=2\left(\rho_{xy}^{U}(x)\frac{\partial\rho_{xy}^{\textrm{U}}(x)}{\partial n}-\rho_{xy}^{L}(x)\frac{\partial\rho_{xy}^{\textrm{L}}(x)}{\partial n}\right)C
\end{split}
\label{nonlinear resistance}
\end{equation}

It is very difficult to say something from Eq. (\ref{linear resistance}) and (\ref{nonlinear resistance}). Now, we suppose a formula for $\rho_{xy}^{U}(x)$ and $\rho_{xy}^{L}(x)$, and simplify the expression. The most straightforward way of modeling the position-dependence is to approximate $\rho_{xy}$ as a linear function of $x$.
\begin{equation}
\begin{split}
\rho_{xy}^{\textrm{U}}(x)&=-\frac{\delta R_{xy}}{L}x+\frac{R_{xy}^{Q}}{2}+\delta R_{xy}\\  
\rho_{xy}^{\textrm{L}}(x)&=-\frac{\delta R_{xy}}{L}x-\frac{R_{xy}^{Q}}{2}
\end{split}  
\end{equation}
We assume that the potential at the source or drain of the sample increase by $\delta R_{xy}I$, namely the intercept.
Then, Eq. (\ref{linear resistance}) and (\ref{nonlinear resistance}) can be simplified as below.
\begin{equation}
\begin{split}
R_{xx}&=-\frac{\delta R_{xy}}{L}d\\
R_{xy}&=R_{xy}^{Q}+\delta R_{xy}
\end{split}
\label{linear resistance model}
\end{equation}

By using this, the potential can be written as below.
\begin{equation}
\begin{split}
\rho_{xy}^{\textrm{U}}(x)&=-\frac{R_{xx}}{d}x+\frac{R_{xy}}{2}-\frac{R_{xx}d}{2L}\\  
\rho_{xy}^{\textrm{L}}(x)&=-\frac{R_{xx}}{d}x-\frac{R_{xy}}{2}-\frac{R_{xx}d}{2L}
\end{split}  
\end{equation}

\begin{equation}
\begin{split}
R_{xx}^{(2)}(\textrm{upper})&=-2\left(\right)dC\\
R_{xy}^{(2)}(\textrm{left})&=2\left(\right)C
\end{split}
\label{nonlinear resistance model}
\end{equation}
